Embedding based on function approximation for large scale image search

The objective of this paper is to design an embedding method that maps local features describing an image (e.g. SIFT) to a higher dimensional representation useful for the image retrieval problem. First, motivated by the relationship between the linear approximation of a nonlinear function in high dimensional space and the stateof-the-art feature representation used in image retrieval, i.e., VLAD, we propose a new approach for the approximation. The embedded vectors resulted by the function approximation process are then aggregated to form a single representation for image retrieval. Second, in order to make the proposed embedding method applicable to large scale problem, we further derive its fast version in which the embedded vectors can be efficiently computed, i.e., in the closed-form. We compare the proposed embedding methods with the state of the art in the context of image search under various settings: when the images are represented by medium length vectors, short vectors, or binary vectors. The experimental results show that the proposed embedding methods outperform existing the state of the art on the standard public image retrieval benchmarks.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> cnn_experiment.tex <==
In this section we further evaluate the proposed F-FAemb when the image is described by a set of CNN features which are state-of-the-art image representation for various computer vision tasks \cite{DBLP:conf/cvpr/RazavianASC14}. Specifically, instead of using set of local SIFT features to describe the image as previous experiments, we extract CNN activations for local patches at multiscale levels. We then take the union of all the patches from the image, regardless of scale. This union set can be considered as local features describing  the image. The same processing (i.e., F-FAemb embedding, whitening, democratic aggregating, rotation normalization, power normalization) is applied on the set of CNN features to produce the single representation. We use the output of the last fully connected layer of the pretrained AlexNet model \cite{jia2014caffe} as CNN features representing for patches. We extract CNN activations at 3 levels. For the first level, we simply take 4096-dimensional CNN activations for the whole image. For the second and the third levels, we extract CNN activations for all $128\times 128$, $64\times64$ patches sampled with a stride of 30 pixels. In order to make the computation of the embedding more efficient, we use PCA to reduce 4096-dimensional features to 45-dimensional features. 

We compare our CNN features-based F-FAemb with the state of the art which use Convolutional Neural Network, deep learning techniques for image retrieval \cite{CKN-paulin,DBLP:conf/cvpr/PerronninL15,DBLP:conf/eccv/GongWGL14,DBLP:conf/cvpr/RazavianASC14}. Note that in this experiment, we follow \cite{DBLP:conf/cvpr/RazavianASC14} which uses the full query images without cropping when evaluating the Oxford5k dataset. 

In \cite{CKN-paulin}, the authors propose a new family of convolutional descriptors for patch presentations based on the Convolutional Kernel Networks (CKN) \cite{DBLP:conf/nips/MairalKHS14} in which the learning is performed in a unsupervised manner, i.e., instead of learning filters by optimizing a loss function as Convolutional Neural Networks, CKN is trained to approximate a particular nonlinear match-kernel, and therefore no labeled data is required. The network is trained on 1M patches from RomePatches dataset \cite{CKN-paulin}. In order to achieve the single representation for an image, they first extract Hessian-Affine regions \cite{mikolajczyk_scale_2004} in the image, feed them to the trained CKN, producing a high dimensional vector (i.e., 41K dimensions) for each patch. The PCA-whitening is applied to reduce these vectors to 1024-dimensional vectors. After that they use VLAD encoding \cite{jegou11d} with 256 centroids to encode the reduced vectors, resulting a very high dimensional (i.e., 262K dimensions) single  VLAD representation. Finally, they apply PCA-whitening to reduce VLAD vector to 4,096 dimensional vector, used for retrieval. 

In \cite{DBLP:conf/cvpr/PerronninL15}, the authors combine Fisher Vector encoding  \cite{DBLP:conf/cvpr/PerronninD07,DBLP:conf/eccv/PerronninSM10} and Deep Neural Network into a single model (FV-DNN) for producing the single representation. Specifically, in their hybrid architecture, the image patches are described by PCA-projected SIFT and color descriptors \cite{Clinchant_xrce}. The projected SIFT and color descriptors are then separately encoded using Fisher encoding. These two Fisher vectors are concatenated; the concatenated vector is subsequently normalized by square-rooting and $l_2$ normalization. The $l_2$ normalized vector is PCA-projected and  $l_2$ normalized again. The resulted vector is fed into supervised layers which is a deep neural network comprising by a sequence of 3 fully connected (hidden) layers, ending by a softmax layer. The model is trained using the ImageNet dataset \cite{ILSVRC15}. The activations of the first supervised hidden layer are used as the image feature in their image retrieval task. In order to boost the performance, they train 8 different models using different random seed initializations. They concatenate the representations produced by 8 models, and reduce the dimension of the concatenated representation with PCA-whitening. 

In \cite{DBLP:conf/eccv/GongWGL14}, the authors propose a CNN-based embedding method named \textit{multiscale orderless pooling (MOP-CNN)}. %This scheme extracts CNN activations for local patches at multiple scales, performs VLAD encoding for the activations at each level separately, and concatenates the encoded vectors, resulting the single representation. 
This scheme first extracts CNN activations for local patches at multiple scales. 
To extract CNN activations for patches, %they use the Caffe implementation pretrained on the ImageNet \cite{ILSVRC15} dataset. 
they use the AlexNet model \cite{jia2014caffe} pretrained on ImageNet dataset \cite{ILSVRC15}. 
They extract CNN activations at three levels. For the first level, they take the 4096-dimensional CNN activations for the whole image. For the remaining two levels, they extract activations for all $128\times 128$ and $64 \times 64$ patches with a stride of 32 pixels, resulting 4096-dimensional activation vectors. In order to make the computation more efficient, they use PCA to reduce CNN activation vectors on the second and the third levels to 500-dimensional vectors. After that they use soft assignment VLAD encoding \cite{DBLP:conf/cvpr/BergamoST13} to encode the reduced vectors of the second level and the third level separately, resulting 50,000-dimensional VLAD vector for each level. They further perform PCA on the VLAD encoded vectors and reduce them to 4096 dimensions. They concatenate the 4096-dimensional CNN feature at the first level and two reduced VLAD encoded vectors at the second and the third level to form a single image representation, and reduce the dimension of the concatenated representation with PCA-whitening. Note that the way we process CNN features differs from \cite{DBLP:conf/eccv/GongWGL14}. Instead encoding the CNN features of levels separately and then concatenating encoded features which causes the dimension of the concatenated vector rapidly increasing, we first make union CNN features of all levels and then perform the encoding only one time. This make the dimension of the final representation independent to the number of levels. 

In \cite{DBLP:conf/cvpr/RazavianASC14}, the authors use the OverFeat model \cite{DBLP:journals/corr/SermanetEZMFL13} pretrained on the ImageNet \cite{ILSVRC15} to extract CNN features. The output 4096-dimensional vector of the first fully connected layer of the network is further post-processing, i.e., $l_2$ normalization, whitening, $l_2$ renormalization, power normalization, and is used as the feature representation for the retrieving. %On Holidays dataset, this single presentation is used the final image representation for the searching. On the Oxford5k dataset in which the interest buildings appear at different locations and scales, they use the spatial search as follows. 
At the retrieval stage, they use the spatial search as follows. 
For each image they extract multiple patches of different sizes at different scales. For each extracted patch they compute its CNN representation. The distance between a query patch and a reference image is defined as the minimum $l_2$ distance between the query patch and respective reference patches. The distance between the query and the reference image is set to the average distance of each query patch to the reference image. %Note that this spatial search is a costly searching and it differs from ours and \cite{CKN-paulin,DBLP:conf/cvpr/PerronninL15,DBLP:conf/eccv/GongWGL14} in which only a single representation is matched per image.

As presented, similar to F-FAemb, all approaches in \cite{CKN-paulin,DBLP:conf/cvpr/PerronninL15,DBLP:conf/eccv/GongWGL14,DBLP:conf/cvpr/RazavianASC14} apply an whitening on the single representation. Thus, for clear presentation, we ignore the \textit{+RN} notation when presenting results of F-FAemb. The mAP of F-FAemb and compared methods is shown in Table \ref{tab:soa_cnn}. The short vector representations of F-FAemb (i.e., when $D<7,245$) is achieved by keeping only first components after the rotation normalization (whitening) step. %It is not surprised that when the CNN features, which is state-of-the-art image representation, is used for FAemb, it significantly boosts the mAP in comparison to the using of SIFT, e.g., at $D=7,245$ the mAP is improved $10.5\%$ and \textcolor{red}{xxx} for Holidays and Oxford5k, respectively. 

%On Holidays dataset, at the same dimension, F-FAemb is on par to FV-DNN\cite{DBLP:conf/cvpr/PerronninL15}, CNN\cite{DBLP:conf/cvpr/RazavianASC14} and considerably improves over MOP-CNN\cite{DBLP:conf/eccv/GongWGL14}, CKN\cite{CKN-paulin}.  

On the Holidays dataset, at the same dimension, F-FAemb slightly improves over FV-DNN\cite{DBLP:conf/cvpr/PerronninL15}, CNN\cite{DBLP:conf/cvpr/RazavianASC14} and considerably improves over MOP-CNN\cite{DBLP:conf/eccv/GongWGL14}, CKN\cite{CKN-paulin}. On the Oxford5k dataset, at the same dimension, F-FAemb is on par to CKN \cite{CKN-paulin} \footnote{The results of CKN\cite{CKN-paulin} on Oxford5k is with cropped queries. According to \cite{CKN-paulin}, the cropped queries achieve better performance than full queries, i.e., the their best mAP with full queries is $55.4$.} while it is lower than CNN\cite{DBLP:conf/cvpr/RazavianASC14}. However it is worth noting that the spatial search used in \cite{DBLP:conf/cvpr/RazavianASC14} is a costly searching as it has two drawbacks. Firstly, all the patch vectors of the image have to be stored. This increases the memory requirements by a factor of $P$ where $P$ is number of extracted patches per image. Secondly, the complexity for computing the distance between two images is increased by a factor of $P^2$. Contrary to \cite{DBLP:conf/cvpr/RazavianASC14}, we only store a single representation per image and compute only one Euclidean distance when comparing two images. 
\begin{table}[!t]
\centering
\small
\caption{Comparison with state-of-the-art CNN / deep learning-based image retrieval.} 
\label{tab:sota_cnn}
\begin{tabular}{|c|c| c c |}
\hline
Method		&$D$ 	 &\multicolumn{2}{|c|}{mAP}\\
			&		 &Holidays 	&Oxford5k	\\ \hline%&Ox105k  \\ \hline
%F-FAemb										&15,525  &00.0  &00.0 \\
F-FAemb										&7,245   &86.0  &59.5 \\\hline%&00.00 \\\hline		
F-FAemb										&4,096   &\textbf{85.4}  &57.8 \\%&00.00 \\ 
CKN\cite{CKN-paulin}			&4,096	 &82.9	&56.5  \\%&00.00 \\(crop, uncrop lower)
FV-DNN\cite{DBLP:conf/cvpr/PerronninL15}	&4,096 	 &84.7  &-     \\%&- \\ 
CNN\cite{DBLP:conf/cvpr/RazavianASC14}		&4,096 	 &84.3  &\textbf{68.0} \\%&- \\ %(uncrop)
\hline
F-FAemb									&2,048  &\textbf{83.5}   &53.4 \\%&00.00 \\ 
MOP-CNN\cite{DBLP:conf/eccv/GongWGL14}	&2,048  &80.2   &- 		\\\hline%&- \\\hline
\end{tabular}
\label{tab:soa_cnn}
\end{table}

==> sota_CNN_retrieval.tex <==
In \cite{CKN-paulin}, the authors propose a new family of convolutional descriptors for patch presentations based on the Convolutional Kernel Networks (CKN) \cite{DBLP:conf/nips/MairalKHS14}. % in which the learning is performed in a unsupervised manner, i.e., instead of learning filters by optimizing a loss function as Convolutional Neural Networks, CKN is trained to approximate a particular nonlinear match-kernel, and therefore no labeled data is required. The network is trained on 1M patches from RomePatches dataset \cite{CKN-paulin}. 
In order to achieve the single representation for an image, they first feed each Hessian-Affine region \cite{mikolajczyk_scale_2004} in the image to a trained CKN, producing a high dimensional vector, which is subsequently reduced by PCA. They then use VLAD encoding \cite{jegou11d} to encode the reduced vectors, resulting a very high dimensional (i.e., 262K dimensions) single  VLAD representation. Finally, they apply PCA-whitening to reduce VLAD vector to 4,096 dimensional vector, used for retrieval. 

In \cite{DBLP:conf/cvpr/PerronninL15}, the authors combine Fisher Vector encoding  \cite{DBLP:conf/cvpr/PerronninD07,DBLP:conf/eccv/PerronninSM10} and Deep Neural Network into a single model (FV-DNN) for producing the single representation. In their architecture, the image patches are described by PCA-projected SIFT and color descriptors \cite{Clinchant_xrce}. The projected SIFT and color descriptors are then separately encoded using Fisher encoding. These two Fisher vectors are concatenated and normalized. The resulted vector is fed into a deep neural network ending by a softmax layer. The activations of the first hidden layer are used as the image feature in their image retrieval task. %In order to boost the performance, they train 8 different models using different random seed initializations. They concatenate the representations produced by 8 models, and reduce the dimension of the concatenated representation with PCA-whitening. 

In \cite{DBLP:conf/eccv/GongWGL14}, the authors propose a CNN-based embedding method named \textit{multiscale orderless pooling (MOP-CNN)}. %This scheme extracts CNN activations for local patches at multiple scales, performs VLAD encoding for the activations at each level separately, and concatenates the encoded vectors, resulting the single representation. 
They used the pretrained AlexNet to extracts CNN activations of the last fully connected layer for local patches at 3 scales (levels) in which first level is whole image. %, resulting 4096-dimensional vectors. 
%To extract CNN activations for patches, they use the AlexNet model \cite{jia2014caffe} pretrained on ImageNet dataset \cite{ILSVRC15}. 
%They extract CNN activations at three levels. For the first level, they take the 4096-dimensional CNN activations for the whole image. For the remaining two levels, they extract activations for all $128\times 128$ and $64 \times 64$ patches with a stride of 32 pixels, resulting 4096-dimensional activation vectors.
The PCA is used to reduce CNN activation vectors on the second and the third levels. After they use the soft assignment VLAD encoding \cite{DBLP:conf/cvpr/BergamoST13} to encode the reduced vectors of these two levels separately.  %They further perform PCA on the VLAD encoded vectors to reduce their dimensions.
 They concatenate the CNN feature at the first level and two 
 %reduced 
 VLAD encoded vectors at the second and the third level to form a single image representation, and reduce the dimension of the concatenated representation with PCA-whitening. Note that the way we process CNN features differs from \cite{DBLP:conf/eccv/GongWGL14}. Instead encoding the CNN features of levels separately and then concatenating encoded features which causes the dimension of the concatenated vector rapidly increasing, we first make union CNN features of all levels and then perform the encoding only one time. This make the dimension of the final representation independent to the number of levels. 

In \cite{DBLP:conf/cvpr/RazavianASC14}, the authors use the OverFeat model \cite{DBLP:journals/corr/SermanetEZMFL13} pretrained on the ImageNet \cite{ILSVRC15} to extract CNN features. The output 4096-dimensional vector of the first fully connected layer of the network is further post-processing, i.e., $l_2$ normalization, whitening, $l_2$ renormalization, power normalization, and is used as the feature representation for the retrieving. %On Holidays dataset, this single presentation is used the final image representation for the searching. On the Oxford5k dataset in which the interest buildings appear at different locations and scales, they use the spatial search as follows. 
At the retrieval stage, they use the spatial search as follows. 
For each image they extract multiple patches of different sizes at different scales. For each extracted patch they compute its CNN representation. The distance between a query patch and a reference image is defined as the minimum $l_2$ distance between the query patch and respective reference patches. The distance between the query and the reference image is set to the average distance of each query patch to the reference image. %Note that this spatial search is a costly searching and it differs from ours and \cite{CKN-paulin,DBLP:conf/cvpr/PerronninL15,DBLP:conf/eccv/GongWGL14} in which only a single representation is matched per image.


==> whiten-aggregate_short.tex <==
Successful instance embedding methods consist of several feature post-processing steps. Adopting the proposed pipeline of~\cite{DBLP:conf/eccv/JegouC12} and followed by others~\cite{DBLP:conf/cvpr/JegouZ14}, we whiten embedded vector $\phi(\x)$, resulting whitened embedded vector $\phi_w(\x)$. 
In~\cite{DBLP:conf/cvpr/JegouZ14}, the authors further indicated that the localization of $\phi_w(\x)$ is improved by discarding some first components associated with the largest eigenvalues. We apply this truncation operation in our experiments. The detail of this truncation operation is presented in section \ref{subsec:compare_4methods}.%

To aggregate set of whitened embedded vectors $\phi_w(\x)$ of the image into a single representation, we use~\textit{democratic aggregation}~\cite{DBLP:conf/cvpr/JegouZ14}. 
Let $\mathcal{X} = \{\x_i\}$ be set of local descriptors described the image, the main idea of democratic aggregation is to find a weight $\lambda_i$ for each $\phi_w(\x_i)$ such that each $\phi_w(\x_i)$ equally contributes to final representation, i.e., $\forall \x_i \in \mathcal{X}$: $\lambda_i \left(\phi_w(\x_i)\right)^T \psi(\mathcal{X}) = 1$
where $\psi(\mathcal{X})$ is the single representation and is defined by: $\psi(\mathcal{X}) = \sum_{\x_i \in \mathcal{X}} \lambda_i \phi_w(\x_i)$.

